Zero-Shot Learning for Requirements Classification: An Exploratory Study

Context: Requirements engineering researchers have been experimenting with machine learning and deep learning approaches for a range of RE tasks, such as requirements classification, requirements tracing, ambiguity detection, and modelling. However, most of today's ML/DL approaches are based on supervised learning techniques, meaning that they need to be trained using a large amount of task-specific labelled training data. This constraint poses an enormous challenge to RE researchers, as the lack of labelled data makes it difficult for them to fully exploit the benefit of advanced ML/DL technologies. Objective: This paper addresses this problem by showing how a zero-shot learning approach can be used for requirements classification without using any labelled training data. We focus on the classification task because many RE tasks can be framed as classification problems. Method: The ZSL approach used in our study employs contextual word-embeddings and transformer-based language models. We demonstrate this approach through a series of experiments to perform three classification tasks: (1)FR/NFR: classification functional requirements vs non-functional requirements; (2)NFR: identification of NFR classes; (3)Security: classification of security vs non-security requirements. Results: The study shows that the ZSL approach achieves an F1 score of 0.66 for the FR/NFR task. For the NFR task, the approach yields F1~0.72-0.80, considering the most frequent classes. For the Security task, F1~0.66. All of the aforementioned F1 scores are achieved with zero-training efforts. Conclusion: This study demonstrates the potential of ZSL for requirements classification. An important implication is that it is possible to have very little or no training data to perform classification tasks. The proposed approach thus contributes to the solution of the long-standing problem of data shortage in RE.

==> Appendices/NFRbinLabels.tex <==
% \usepackage{caption}
% \usepackage{booktabs}
% \usepackage{vcell}


\begin{table}
\centering
\caption{Label configurations for the remaining NFR classes for Task NFR, binary classification case (continued to table for Table \ref{tab:labelsNFRbinary}).}
  \resizebox{1\textwidth}{!}{
 \label{tab:appendixNFRbinLabels}
\begin{tabular}{llll} 
\toprule
\vcell{\textbf{Label Abbr.}}            & \vcell{\textbf{Label Configuration}}                                                                         & \vcell{\textbf{NFR Label}}                                                                                                                                                                                                                                                                                                                                                                                                            & \vcell{\textbf{"Other" Label}}                                                                                                                                                                                                                       \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\ 
\hline
\vcell{\textbf{\textit{Performance}}}   & \vcell{}                                                                                                     & \vcell{}                                                                                                                                                                                                                                                                                                                                                                                                                              & \vcell{}                                                                                                                                                                                                                                             \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{PE\_A}}} & \vcell{Original 1}                                                                                           & \vcell{"performance"}                                                                                                                                                                                                                                                                                                                                                                                                                 & \vcell{"not about performance"}                                                                                                                                                                                                                      \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{PE\_B}}} & \vcell{Expert curated}                                                                                       & \vcell{"periodic execution or efficacy performance"}                                                                                                                                                                                                                                                                                                                                                                                  & \vcell{"not about periodic execution or efficacy performance"}                                                                                                                                                                                       \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{PE\_C}}} & \vcell{\begin{tabular}[b]{@{}l@{}}Word Embedding \\(selected from top 20 words)\end{tabular}}                & \vcell{\begin{tabular}[b]{@{}l@{}}"throughput, reliability, scalability, responsiveness, efficiency, \\workload, benchmark, latency, speed, improvement, or accuracy"\end{tabular}}                                                                                                                                                                                                                                                   & \vcell{\begin{tabular}[b]{@{}l@{}}"not about throughput, reliability, scalability, responsiveness,\\~efficiency, workload, benchmark, latency, speed, improvement,\\~or accuracy"\end{tabular}}                                                      \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{PE\_D}}} & \vcell{\begin{tabular}[b]{@{}l@{}}Word Embedding \\(selected from top 20 words) \\+ Original 2\end{tabular}} & \vcell{\begin{tabular}[b]{@{}l@{}}"throughput, reliability, scalability, responsiveness, efficiency,\\~workload, benchmark, latency, speed, improvement, or accuracy"\end{tabular}}                                                                                                                                                                                                                                                   & \vcell{\begin{tabular}[b]{@{}l@{}}"usability, security, operational, look \& feel, legal, fault \& tolerance,\\~maintainability, scalability, availability, or portability"\end{tabular}}                                                            \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{PE\_E}}} & \vcell{\begin{tabular}[b]{@{}l@{}}Word Embedding \\(selected from top 50 words) \\+ Original 2\end{tabular}} & \vcell{\begin{tabular}[b]{@{}l@{}}"throughput, reliability, scalability, responsiveness, efficiency, \\workload, benchmark, latency, speed, improvement, accuracy,\\~achieve, tuning, bottleneck, better, high, optimize, effectiveness, \\low, enhances, reducing, incresaed, quality, faster, or degrades"\end{tabular}}                                                                                                            & \vcell{\begin{tabular}[b]{@{}l@{}}"usability, security, operational, look \& feel, legal, fault \& tolerance, \\maintainability, scalability, availability, or portability"\end{tabular}}                                                            \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\ 
\hline
\vcell{\textbf{\textit{Operational}}}   & \vcell{}                                                                                                     & \vcell{}                                                                                                                                                                                                                                                                                                                                                                                                                              & \vcell{}                                                                                                                                                                                                                                             \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{O\_A}}}  & \vcell{Original 1}                                                                                           & \vcell{"operational"}                                                                                                                                                                                                                                                                                                                                                                                                                 & \vcell{"not about operational"}                                                                                                                                                                                                                      \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{O\_B}}}  & \vcell{Expert curated}                                                                                       & \vcell{"working, running, connecting, interfacing, or operative environment"}                                                                                                                                                                                                                                                                                                                                                         & \vcell{\begin{tabular}[b]{@{}l@{}}"not about working, running, connecting, interfacing, \\or operative environment"\end{tabular}}                                                                                                                    \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{O\_C}}}  & \vcell{\begin{tabular}[b]{@{}l@{}}Word Embedding\\(selected from top 20 words)\end{tabular}}                 & \vcell{"environmental, organizational, coordination, systemic, or logistics"}                                                                                                                                                                                                                                                                                                                                                         & \vcell{\begin{tabular}[b]{@{}l@{}}"not about environmental, organizational, coordination, \\systemic, or logistics"\end{tabular}}                                                                                                                    \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{O\_D}}}  & \vcell{\begin{tabular}[b]{@{}l@{}}Word Embedding \\(selected from top 20 words) \\+ Original 2\end{tabular}} & \vcell{"environmental, organizational, coordination, systemic, or logistics"}                                                                                                                                                                                                                                                                                                                                                         & \vcell{\begin{tabular}[b]{@{}l@{}}"usability, security, performance, look \& feel, legal, fault \& tolerance, \\maintainability, scalability, availability, or portability"\end{tabular}}                                                            \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{O\_E}}}  & \vcell{\begin{tabular}[b]{@{}l@{}}Word Embedding \\(selected from top 50 words)\\~+ Original 2\end{tabular}} & \vcell{\begin{tabular}[b]{@{}l@{}}"environmental, organizational, coordination, systemic, logistics,\\~coordination, or automation"\end{tabular}}                                                                                                                                                                                                                                                                                     & \vcell{\begin{tabular}[b]{@{}l@{}}"usability, security, performance, look \& feel, legal, fault \& tolerance, \\maintainability, scalability, availability, or portability"\end{tabular}}                                                            \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\ 
\hline
\vcell{\textbf{\textit{Look \& feel}}}  & \vcell{}                                                                                                     & \vcell{}                                                                                                                                                                                                                                                                                                                                                                                                                              & \vcell{}                                                                                                                                                                                                                                             \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{LF\_A}}} & \vcell{Original 1}                                                                                           & \vcell{"Look  feel"}                                                                                                                                                                                                                                                                                                                                                                                                                  & \vcell{"not about Look  feel"}                                                                                                                                                                                                                       \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{LF\_B}}} & \vcell{Expert curated}                                                                                       & \vcell{"appearance, interface, look  feel"}                                                                                                                                                                                                                                                                                                                                                                                           & \vcell{"not about appearance, interface, look  feel"}                                                                                                                                                                                                \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{LF\_C}}} & \vcell{\begin{tabular}[b]{@{}l@{}}Word Embedding\\(selected from top 20 words)\end{tabular}}                 & \vcell{\begin{tabular}[b]{@{}l@{}}"graphical, gui, ui, widget, interaction, habit, prefer, comfortable, friendly, \\feeling, experience, or familiar"\end{tabular}}                                                                                                                                                                                                                                                                   & \vcell{\begin{tabular}[b]{@{}l@{}}" not about graphical, gui, ui, widget, interaction, habit, prefer, \\comfortable, friendly, feeling, experience, or familiar"\end{tabular}}                                                                       \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{LF\_D}}} & \vcell{\begin{tabular}[b]{@{}l@{}}Word Embedding\\(selected from top 20 words) \\+ Original 2\end{tabular}}  & \vcell{\begin{tabular}[b]{@{}l@{}}"graphical, gui, ui, widget, interaction, habit, prefer, comfortable, friendly,\\~feeling, experience, or familiar"\end{tabular}}                                                                                                                                                                                                                                                                   & \vcell{\begin{tabular}[b]{@{}l@{}}"usability, security, operational, performance, fault \& tolerance,\\~legal, maintainability, scalability, availability, or portability"\end{tabular}}                                                             \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{LF\_E}}} & \vcell{\begin{tabular}[b]{@{}l@{}}Word Embedding \\(selected from top 50 words) \\+ Original 2\end{tabular}} & \vcell{\begin{tabular}[b]{@{}l@{}}"graphical, gui, ui, widget, interaction, habit, prefer, comfortable, friendly,\\~feeling, experience, familiar, desire, customize, intent, disability, \\or impression"\end{tabular}}                                                                                                                                                                                                              & \vcell{\begin{tabular}[b]{@{}l@{}}"usability, security, operational, performance, fault \& tolerance, \\legal, maintainability, scalability, availability, or portability"\end{tabular}}                                                             \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\ 
\hline
\vcell{\textbf{\textit{Legal}}}         & \vcell{}                                                                                                     & \vcell{}                                                                                                                                                                                                                                                                                                                                                                                                                              & \vcell{}                                                                                                                                                                                                                                             \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{L\_A}}}  & \vcell{Original 1}                                                                                           & \vcell{"legal"}                                                                                                                                                                                                                                                                                                                                                                                                                       & \vcell{"not about legal"}                                                                                                                                                                                                                            \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{L\_B}}}  & \vcell{Expert curated}                                                                                       & \vcell{"legal, law, or rules"}                                                                                                                                                                                                                                                                                                                                                                                                        & \vcell{"not about legal, law, or rules"}                                                                                                                                                                                                             \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{L\_C}}}  & \vcell{\begin{tabular}[b]{@{}l@{}}Word Embedding \\(selected from top 20 words)\end{tabular}}                & \vcell{\begin{tabular}[b]{@{}l@{}}"liability, litigation, jurisdiction, regulation, copyright, legislation, \\enforcement, governmental, directive, civil, right, patentability,\\~claim, violate, infringement, or counsel"\end{tabular}}                                                                                                                                                                                            & \vcell{\begin{tabular}[b]{@{}l@{}}"not about liability, litigation, jurisdiction, regulation, copyright,\\~legislation, enforcement, governmental, directive,civil, right,\\~patentability, claim, violate, infringement, or counsel"\end{tabular}}  \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{L\_D}}}  & \vcell{\begin{tabular}[b]{@{}l@{}}Word Embedding \\(selected from top 20 words) \\+ Original 2\end{tabular}} & \vcell{\begin{tabular}[b]{@{}l@{}}"liability, litigation, jurisdiction, regulation, copyright, legislation,\\enforcement, governmental, directive,civil, right, patentability,\\~claim, violate, infringement, or counsel"\end{tabular}}                                                                                                                                                                                              & \vcell{\begin{tabular}[b]{@{}l@{}}"usability, security, operational, performance, look \& feel,\\~fault \& tolerance, maintainability, scalability, availability, \\or portability"\end{tabular}}                                                    \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\vcell{\textbf{\textit{L\_E}}}  & \vcell{\begin{tabular}[b]{@{}l@{}}Word Embedding \\(selected from top 50 words) \\+ Original 2\end{tabular}} & \vcell{\begin{tabular}[b]{@{}l@{}}"liability, litigation, jurisdiction, regulation, copyright, legislation,\\~enforcement, governmental, directive,civil, right, patentability, \\claim, violate, infringement,~~counsel, holder, dispute, illegal, judicial,\\~ruling, agreement, ownership, comply, authority, law, accountability, \\abuse, intellectual, obligation, invention,~court, ethical, concern, or policy"\end{tabular}} & \vcell{\begin{tabular}[b]{@{}l@{}}"usability, security, operational, performance, look \& feel, \\fault \& tolerance, maintainability, scalability, availability, \\or portability"\end{tabular}}                                                    \\[-\rowheight]
\printcelltop                           & \printcelltop                                                                                                & \printcelltop                                                                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                                                        \\
\bottomrule
\end{tabular}
}
\end{table}

\addtocounter{table}{-1}


% \usepackage{caption}
% \usepackage{booktabs}


\begin{table}
\centering
\caption{Continued }
  \resizebox{1\textwidth}{!}{
\begin{tabular}{llll} 
\toprule
\textbf{Label Abbr.}               & \textit{\textbf{Label Configuration}}                                                                & \textit{\textbf{NFR Label}}                                                                                                                                                                                                                                           & \textit{\textbf{"Other" Label}}                                                                                                                                                                                                                                                  \\ 
\hline
\textbf{\textit{Fault tolerance}}  &                                                                                                      &                                                                                                                                                                                                                                                                       &                                                                                                                                                                                                                                                                                  \\
\textbf{\textit{FT\_A}}    & Original 1                                                                                           & "fault  tolerance"                                                                                                                                                                                                                                                    & "not about fault  tolerance"                                                                                                                                                                                                                                                     \\
\textbf{\textit{FT\_B}}    & Expert curated                                                                                       & "system recovery  fault tolerance"                                                                                                                                                                                                                                    & "not about system recovery  fault tolerance"                                                                                                                                                                                                                                     \\
\textbf{\textit{FT\_C}}    & \begin{tabular}[c]{@{}l@{}}Word Embedding \\(selected from top 20 words)\end{tabular}                & \begin{tabular}[c]{@{}l@{}}"tolerance, failure, tolerant, byzantine, deadlock, exploiting, \\reliability, isolation, fault, guarantee, or dependable"\end{tabular}                                                                                                    & \begin{tabular}[c]{@{}l@{}}"not about tolerance, failure, tolerant, byzantine, deadlock, exploiting, reliability,\\~isolation, fault, guarantee, dependable, countermeasure, resilience, defensive,\\~corruption, weakness, malfunction, robustness, or stability"\end{tabular}  \\
\textbf{\textit{FT\_D}}    & \begin{tabular}[c]{@{}l@{}}Word Embedding \\(selected from top 20 words) \\+ Original 2\end{tabular} & \begin{tabular}[c]{@{}l@{}}"tolerance, failure, tolerant, byzantine, deadlock, exploiting,\\~reliability, isolation, fault, guarantee, or dependable"\end{tabular}                                                                                                    & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, performance, look \& feel, legal, maintainability, \\scalability, availability, or portability"\end{tabular}                                                                                                       \\
\textbf{\textit{FT\_E}}    & \begin{tabular}[c]{@{}l@{}}Word Embedding \\(selected from top 50 words) \\+ Original 2\end{tabular} & \begin{tabular}[c]{@{}l@{}}"tolerance, failure, tolerant, byzantine, deadlock, exploiting,\\~reliability, isolation, fault, guarantee, dependable, countermeasure, \\resilience, defensive, corruption, weakness, malfunction, robustness, or stability"\end{tabular} & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, performance, look \& feel, legal, maintainability,\\~scalability, availability, or portability"\end{tabular}                                                                                                       \\ 
\hline
\textbf{\textit{Maintainability~}} &                                                                                                      &                                                                                                                                                                                                                                                                       &                                                                                                                                                                                                                                                                                  \\
\textbf{\textit{MN\_A}}    & Original 1                                                                                           & "maintainability"                                                                                                                                                                                                                                                     & "not about maintainability"                                                                                                                                                                                                                                                      \\
\textbf{\textit{MN\_B}}    & Expert curated                                                                                       & "maintaining, fixing, running or updating"                                                                                                                                                                                                                            & "not about maintaining, fixing, running or updating"                                                                                                                                                                                                                             \\
\textbf{\textit{MN\_C}}    & \begin{tabular}[c]{@{}l@{}}Word Embedding\\(selected from top 20 words)\end{tabular}                 & "adaptability, effectiveness, agility, preventive, or dependability"                                                                                                                                                                                                  & "not about adaptability, effectiveness, agility, preventive, or dependability"                                                                                                                                                                                                   \\
\textbf{\textit{MN\_D}}    & \begin{tabular}[c]{@{}l@{}}Word Embedding \\(selected from top 20 words) \\+ Original 2\end{tabular} & "adaptability, effectiveness, agility, preventive, or dependability"                                                                                                                                                                                                  & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, performance, look \& feel, legal, fault \& tolerance, \\scalability, availability, or portability"\end{tabular}                                                                                                    \\
\textbf{\textit{MN\_E}}    & \begin{tabular}[c]{@{}l@{}}Word Embedding \\(selected from top 50 words) \\+ Original 2\end{tabular} & \begin{tabular}[c]{@{}l@{}}"adaptability, effectiveness, agility, preventive, dependability, \\correcting, reuse, defect, mitigation, validated, resilience, achievable, \\remedy, assessing, or maintaining"\end{tabular}                                            & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, performance, look \& feel, legal, fault \& tolerance, \\scalability, availability, or portability"\end{tabular}                                                                                                    \\ 
\hline
\textbf{\textit{Scalability}}      &                                                                                                      &                                                                                                                                                                                                                                                                       &                                                                                                                                                                                                                                                                                  \\
\textbf{\textit{SC\_A}}    & Original 1                                                                                           & "scalability"                                                                                                                                                                                                                                                         & "not about scalability"                                                                                                                                                                                                                                                          \\
\textbf{\textit{SC\_B}}    & Expert curated                                                                                       & "scalable, increasable or developable"                                                                                                                                                                                                                                & "not about scalable, increasable or developable"                                                                                                                                                                                                                                 \\
\textbf{\textit{SC\_C}}    & \begin{tabular}[c]{@{}l@{}}Word Embedding \\(selected from top 20 words)\end{tabular}                & "flexibility, workload, efficiency, or optimize"                                                                                                                                                                                                                      & "not about flexibility, workload, efficiency, or optimize"                                                                                                                                                                                                                       \\
\textbf{\textit{SC\_D}}    & \begin{tabular}[c]{@{}l@{}}Word Embedding \\(selected from top 20 words) \\+ Original 2\end{tabular} & "flexibility, workload, efficiency, or optimize"                                                                                                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, performance, look \& feel, legal, fault \& tolerance, \\maintainability, availability, or portability"\end{tabular}                                                                                                \\
\textbf{\textit{SC\_E}}    & \begin{tabular}[c]{@{}l@{}}Word Embedding \\(selected from top 50 words) \\+ Original 2\end{tabular} & \begin{tabular}[c]{@{}l@{}}"flexibility, workload, efficiency, optimize, caching, improvement,\\~robust, overhead, adaptability, scalable, or increased"\end{tabular}                                                                                                 & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, performance, look \& feel, legal, fault \& tolerance,\\~maintainability, availability, or portability"\end{tabular}                                                                                                \\ 
\hline
\textbf{\textit{Availability~}}    &                                                                                                      &                                                                                                                                                                                                                                                                       &                                                                                                                                                                                                                                                                                  \\
\textbf{\textit{A\_A}}     & Original 1                                                                                           & "availability"                                                                                                                                                                                                                                                        & "not about availability"                                                                                                                                                                                                                                                         \\
\textbf{\textit{A\_B}}     & Expert curated                                                                                       & "avaliable or timely achievable"                                                                                                                                                                                                                                      & "not about avaliable or timely achievable"                                                                                                                                                                                                                                       \\
\textbf{\textit{A\_C}}     & \begin{tabular}[c]{@{}l@{}}Word Embedding \\(selected from top 20 words)\end{tabular}                & "reliability, dependability, resilience"                                                                                                                                                                                                                              & "not about reliability, dependability, resilience"                                                                                                                                                                                                                               \\
\textbf{\textit{A\_D}}     & \begin{tabular}[c]{@{}l@{}}Word Embedding \\(selected from top 20 words)\\+ Original 2\end{tabular}  & "reliability, dependability, resilience"                                                                                                                                                                                                                              & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, performance, look \& feel, legal, fault \& tolerance,\\~maintainability, scalability, or portability"\end{tabular}                                                                                                 \\
\textbf{\textit{A\_E}}     & \begin{tabular}[c]{@{}l@{}}Word Embedding \\(selected from top 50 words) \\+ Original 2\end{tabular} & \begin{tabular}[c]{@{}l@{}}"reliability, dependability, resilience, flexibility, accountability, \\ensur, disruption, timely, or standby"\end{tabular}                                                                                                                & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, performance, look \& feel, legal, fault~~\& tolerance,\\~maintainability, scalability, or portability"\end{tabular}                                                                                                \\
\bottomrule
\end{tabular}
}
\end{table}

==> Appendices/NFRmultiLabels.tex <==
% \usepackage{caption}
% \usepackage{booktabs}


\begin{table}
\centering
\caption{Label configurations for all the NFR classes for the multi-class and multi-label classification sub-tasks in Task NFR (cf. Table \ref{tab:labelsNFRmulti})}
 \label{tab:appendixNFRmultiLabels}
  \resizebox{1\textwidth}{!}{
\begin{tabular}{lll} 
\toprule
\textbf{Label Abbr.}          & \textbf{Label Configuration}                                                          & \textbf{List of Labels}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ 
\hline
\textbf{\textit{MultiNFR\_A}} & Original                                                                              & {[}"usability", "security", "performance", "operational", "look \& feel", "legal", "fault tolerance", "maintainability", scalability" availability"]                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\
\textbf{\textit{MultiNFR\_B}} & Expert curated                                                                        & \begin{tabular}[c]{@{}l@{}}{[}"instructive, easy, helpful, useful, learnable, explainable, affordable, intuitive, or understandable",\\"security, authorization, or protection", "periodic execution or efficacy performance",\\"working, running, connecting, interfacing, or operative environment",\\"appearance, interface, look \& feel", "legal, law, or rules", "system recovery \& fault tolerance",\\"maintaining, fixing, running or updating", "scalable, increasable or developable", "avaliable or timely achievable"]\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\
\textbf{\textit{MultiNFR\_C}} & \begin{tabular}[c]{@{}l@{}}Word Embedding \\(selected from top 20 words)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}"accessibility, aesthetic, contextual, experience, satisfaction, HCI, UX, questionnaire, ease, or ergonomics" ,\\"vulnerability, securing. protecting, protection, cybersecurity, assurance, cyber, countermeasure, threat, \\privacy, authentication, prevention, or confidentiality",~"throughput, reliability, scalability, responsiveness, \\efficiency, workload, benchmark, latency, speed, improvement, or accuracy", "environmental, organizational, \\coordination, systemic, or logistics", "graphical, gui, ui, widget, interaction, habit, prefer, comfortable,\\~friendly, feeling, experience, or familiar", "liability, litigation, jurisdiction, regulation, copyright, legislation, \\enforcement, governmental, directive,civil, right, patentability, claim, violate, infringement, or counsel",\\"tolerance, failure, tolerant, byzantine, deadlock, exploiting, reliability, isolation, fault, guarantee, or dependable",\\"adaptability, effectiveness, agility, preventive, or dependability", "flexibility, workload, efficiency, or optimize",\\"reliability, dependability, resilience"]\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\
\textbf{\textit{MultiNFR\_D}} & \begin{tabular}[c]{@{}l@{}}Word Embedding\\~(selected from top 50 words)\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}"accessibility, aesthetic, contextual, experience, satisfaction, HCI, UX, questionnaire, ease, \\ergonomics, designer, evaluate, multimodal, practitioner, prototyping, preference, personalization,\\~suitability, focus, clarity, responsiveness, judgement, feel, or helpful" , "vulnerability, security, \\protection, cybersecurity, assurance, countermeasure, threat, privacy, authentication, prevention, \\confidentiality, trusted, intrusion, compromise, safety, insecure, defensive, breach, proactive, tampering, \\penetration, policy, phishing, vulnerable, authorization, dependability, or certification",\\"throughput, reliability, scalability, responsiveness, efficiency, workload, benchmark, latency, \\speed, improvement, accuracy, achieve, tuning, bottleneck, better, high, optimize, effectiveness, \\low, enhances, reducing, incresaed, quality, faster, or degrades", "environmental, organizational, \\coordination, systemic, logistics, coordination, or automation",~"graphical, gui, ui, widget, interaction, \\habit, prefer, comfortable, friendly, feeling, experience, familiar, desire, customize, intent, disability, or impression",\\"liability, litigation, jurisdiction, regulation, copyright, legislation, enforcement, governmental, directive,civil, right,\\~patentability, claim, violate, infringement, counsel, holder, dispute, illegal, judicial, ruling, agreement, ownership,\\~comply, authority, law, accountability, abuse, intellectual, obligation, invention, court, ethical, concern, or policy",\\"tolerance, failure, tolerant, byzantine, deadlock, exploiting, reliability, isolation, fault, guarantee, dependable, \\countermeasure, resilience, defensive, corruption, weakness, malfunction, robustness, or stability",\\"adaptability, effectiveness, agility, preventive, dependability, correcting, reuse, defect, mitigation, validated,\\~resilience, achievable, remedy, assessing, or maintaining",\\"flexibility, workload, efficiency, optimize, caching, improvement, robust, overhead, adaptability, scalable, or increased",\\"reliability, dependability, resilience, flexibility, accountability, ensur, disruption, timely, or standby"]\end{tabular}  \\
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/BestLabels4NFRBinary.tex <==
% \usepackage{booktabs}
% \usepackage{vcell}


\begin{table}
\centering
\caption{Tracking best performance scores (Weighted F1)  per LM and Label groups for task B: the binary classification of non-functional requirements. (x) refers to none. Letter code refers to the NFR class abbreviation in the dataset. (*) indicates a matched F1 score.}
\label{tab:bestlabels4NFRbinary}
 \resizebox{1\textwidth}{!}{
\begin{tabular}{l|c|c|l|l|l} 
\toprule
\vcell{\textbf{\textit{LM vs Label Group}}} & \vcell{\textbf{(NFR)\_A}} & \vcell{\textbf{(NFR)\_B}} & \vcell{\textbf{(NFR)\_C}}          & \vcell{\textbf{(NFR)\_D}} & \vcell{\textbf{(NFR)\_E}}          \\[-\rowheight]
\printcelltop                              & \printcelltop             & \printcelltop             & \printcelltop                      & \printcelltop             & \printcelltop                      \\ 
\hline
\vcell{\textbf{Sbert}}                     & \vcell{x}                 & \vcell{x}                 & \multicolumn{1}{c|}{\vcell{x}}     & \vcell{O, FT, L, LF, SC}  & \vcell{SE, US, PE, A, MN}          \\[-\rowheight]
\printcelltop                              & \printcelltop             & \printcelltop             & \multicolumn{1}{c|}{\printcelltop} & \printcelltop             & \printcelltop                      \\ 
\hline
\vcell{\textbf{AllMini}}                   & \vcell{x}                 & \vcell{A}                 & \multicolumn{1}{c|}{\vcell{x}}     & \vcell{SE, US, LF*}       & \vcell{O, PE, FT, L, LF*, SC, MN}  \\[-\rowheight]
\printcelltop                              & \printcelltop             & \printcelltop             & \multicolumn{1}{c|}{\printcelltop} & \printcelltop             & \printcelltop                      \\ 
\hline
\vcell{\textbf{Bert4RE}}                   & \vcell{x}                 & \vcell{x}                 & \vcell{SE, O, L, SC}               & \vcell{US, PE, LF}        & \vcell{FT, MN, A}                  \\[-\rowheight]
\printcelltop                              & \printcelltop             & \printcelltop             & \printcelltop                      & \printcelltop             & \printcelltop                      \\ 
\hline
\vcell{\textbf{SObert}}                    & \vcell{x}                 & \vcell{US}                & \vcell{SE, O, PE, LF}              & \vcell{A, L, SC}          & \vcell{FT, MN}                     \\[-\rowheight]
\printcelltop                              & \printcelltop             & \printcelltop             & \printcelltop                      & \printcelltop             & \printcelltop                      \\
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/CompareNFRbinary.tex <==
% \usepackage[normalem]{ulem}
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}
\centering
\caption{Binary classification results obtained from \textit{Task NFR} compared to the results obtained by K\&M and NoRBERT. Bold values indicate the best performance results. Underlined values refer to the best performance rates with the ZSL classifier. The last column \textbf{A} represents the overall weighted F1 score across classes. Only top 4 NFR classes are considered.}
\label{tab:compareNFRbinary}
\resizebox{1\textwidth}{!}{
\begin{tabular}{c|l|rrr|rrr|rrr|rrr|c} 
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Approach(parameters)}}}                                                                                                              & \multicolumn{3}{c|}{\textbf{US (67)}}                                                              & \multicolumn{3}{c|}{\textbf{SE (66)}}                                                              & \multicolumn{3}{c|}{\textbf{O (62)}}                                                               & \multicolumn{3}{c|}{\textbf{PE (54)}}                                                              & \multicolumn{1}{r}{\multirow{2}{*}{\textbf{~wF1}}}  \\ 
\cline{3-14}
\multicolumn{2}{c|}{}                                                                                                                                                            & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{r}{}                                \\ 
\hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}10-fold \\cross val.\\on Top-4 \\NFR~(249)\end{tabular}} & K\&M(w/o features selection)                                                 & 0.81                           & \textbf{0.85}                  & 0.82                             & 0.91                           & \textbf{0.90}                  & 0.88                             & 0.72                           & \textbf{0.75}                  & 0.73                             & \textbf{0.93}                  & \textbf{0.90}                  & \textbf{0.90}                    & \textbf{0.83}                                       \\
                                                                                                    & K\&M(best 50 features)                                                       & 0.70                           & 0.57                           & 0.61                             & 0.81                           & 0.77                           & 0.74                             & 0.78                           & 0.50                           & 0.57                             & 0.87                           & 0.57                           & 0.67                             & 0.65                                                \\
                                                                                                    & K\&M(best 500 features)                                                      & 0.80                           & 0.71                           & 0.74                             & 0.74                           & 0.81                           & 0.74                             & 0.72                           & 0.73                           & 0.71                             & 0.87                           & 0.81                           & 0.82                             & 0.75                                                \\ 
\cline{2-15}
                                                                                                    & NoRBERT(base + ep.10)                                                      & 0.81                           & 0.69                           & 0.74                             & \textbf{0.93}                  & 0.82                           & 0.87                             & 0.80                           & 0.53                           & 0.64                             & 0.88                           & 0.80                           & 0.83                             & 0.77                                                \\
                                                                                                    & NoRBERT(base + ep.10 - OS\tablefootnote{OS refers to Oversampling technique for randomly selecting data from the minority class by adding them to the training dataset Sampling })                                                 & 0.78                           & 0.70                           & 0.74                             & 0.90                           & 0.86                           & 0.88                             & 0.88                           & 0.71                           & \textbf{0.79}                    & 0.88                           & 0.80                           & 0.83                             & 0.81                                                \\
                                                                                                    & NoRBERT(large+OS+ES\tablefootnote{ES refers Early Stopping, a feature that enables the model training to be automatically stopped when a selected metric (e.g., F1) has stopped improving})                                                       & \textbf{0.89}                  & 0.70                           & \textbf{0.78}                    & 0.89                           & 0.89                           & \textbf{0.89}                    & \textbf{0.90}                  & 0.71                           & \textbf{0.79}                    & 0.88                           & 0.81                           & 0.85                             & \textbf{0.83}                                       \\ 
\hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Test Top-4 \\NFR (249) \\w/o training~\end{tabular}}     & ZSL(Sbert + (NFR)\_D)                                                      & 0.77                           & 0.78                           & 0.78                             & 0.72                           & 0.71                           & 0.72                             & 0.68                           & 0.72                           & 0.70                             & 0.80                           & 0.67                           & 0.70                             & 0.72                                                \\
                                                                                                    & \textbf{ZSL(Sbert + (NFR)\_E)}                                             & \textbf{\uline{0.81}}          & \textbf{\uline{0.82}}          & \textbf{\uline{0.80}}            & 0.76                           & 0.78                           & 0.75                             & 0.68                           & 0.63                           & 0.65                             & 0.78                           & \textbf{\uline{0.78}}          & \textbf{\uline{0.78}}            & \textbf{\uline{0.74}}                               \\
                                                                                                    & ZSL(AllMini + (NFR)\_B)                                                    & 0.54                           & 0.35                           & 0.35                             & 0.73                           & 0.73                           & 0.73                             & 0.71                           & 0.65                           & 0.67                             & 0.80                           & 0.70                           & \textbf{\uline{0.78}}            & 0.62                                                \\
                                                                                                    & \textbf{ZSL(AllMini + (NFR)\_D)}                                           & 0.75                           & 0.75                           & 0.75                             & \textbf{\uline{0.84}}          & \textbf{\uline{0.84}}          & \textbf{\uline{0.84}}            & 0.65                           & 0.55                           & 0.58                             & \textbf{\uline{0.81}}          & 0.69                           & 0.71                             & 0.72                                                \\
                                                                                                    & \begin{tabular}[c]{@{}l@{}}\textbf{ZSL(BERT4RE + (NFR)\_C)}\\\end{tabular} & 0.52                           & 0.43                           & 0.46                             & 0.62                           & 0.65                           & 0.63                             & \textbf{\uline{0.72}}          & \textbf{\uline{0.73}}          & \textbf{\uline{0.72}}            & 0.68                           & 0.41                           & 0.43                             & 0.56                                                \\
                                                                                                    & ZSL(BERT4RE + (NFR)\_D)                                                    & 0.54                           & 0.42                           & 0.45                             & 0.56                           & 0.70                           & 0.61                             & 0.63                           & 0.41                           & 0.42                             & 0.60                           & 0.46                           & 0.51                             & 0.50                                                \\
                                                                                                    & ZSL(SObert + (NFR)\_B)                                                     & 0.55                           & 0.51                           & 0.53                             & 0.81                           & 0.74                           & 0.63                             & 0.65                           & \textbf{\uline{0.73}}          & 0.67                             & 0.61                           & \textbf{\uline{0.78}}          & 0.68                             & 0.62                                                \\
                                                                                                    & ZSL(SObert + (NFR)\_C)                                                     & 0.51                           & 0.32                           & 0.30                             & 0.66                           & 0.53                           & 0.56                             & 0.71                           & 0.74                           & 0.71                             & 0.61                           & 0.55                           & 0.58                             & 0.53                                                \\
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/CompareNFRmulti.tex <==
% \usepackage[normalem]{ulem}
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}
\centering
\caption{Multi-class classification results obtained from \textit{Task NFR} compared to the results obtained by Kurtanović  Maalej (2017) and Hey et al. (2020). Bold values indicate the best performance results. Underlined values refer to the best performance rates with the ZSL classifier. The last column \textbf{A} represents the overall weighted F1 score across classes. Only top 4 NFR classes are considered.}
\label{tab:compareNFRmulti}
\resizebox{1\textwidth}{!}{
\begin{tabular}{c|l|ccc|ccc|ccc|ccc|c} 
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{ Approach (parameters)}}}                                                                      & \multicolumn{3}{c|}{\textbf{US (67)}}                                  & \multicolumn{3}{c|}{\textbf{SE (66)}}                         & \multicolumn{3}{c|}{\textbf{O (62)}}                                  & \multicolumn{3}{c|}{\textbf{PE (54)}}                                 & \multirow{2}{*}{\textbf{A}}  \\ 
\cline{3-14}
\multicolumn{2}{c|}{}                                                                                                                      & \multicolumn{1}{l}{\textbf{P}} & \textbf{R}            & \textbf{F1}   & \textbf{P}    & \textbf{R}            & \textbf{F1}           & \textbf{P}            & \textbf{R}            & \textbf{F1}           & \textbf{P}            & \textbf{R}            & \textbf{F1}           &                              \\ 
\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}10-fold\\~cross val. \\on Top-4~\\NFR (249)\end{tabular}} & K\&M(word features)                   & 0.65                           & 0.82                  & 0.70          & 0.81          & 0.77                  & 0.75                  & 0.81                  & \textbf{0.86}         & \textbf{0.82}         & 0.86                  & \textbf{0.81}         & 0.80                  & 0.76                         \\
                                                                                                     & K\&M(best 50 features)                & 0.49                           & 0.68                  & 0.55          & 0.60          & 0.50                  & 0.39                  & 0.42                  & 0.47                  & 0.33                  & 0.85                  & 0.53                  & 0.63                  & 0.47                         \\
                                                                                                     & K\&M(best 500 features)               & 0.70                           & 0.66                  & 0.64          & 0.64          & 0.53                  & 0.56                  & 0.47                  & 0.62                  & 0.51                  & 0.81                  & 0.74                  & 0.76                  & 0.61                         \\
                                                                                                     & NoRBERT(base+ep.32)                 & 0.78                           & \textbf{0.84}         & 0.81          & 0.89          & 0.85                  & 0.87                  & 0.79                  & 0.73                  & 0.76                  & 0.88                  & 0.78                  & 0.82                  & 0.82                         \\
                                                                                                     & NoRBERT(large+ep.32)                & \textbf{0.86}                  & 0.82                  & \textbf{0.84} & \textbf{0.91} & \textbf{0.91}         & \textbf{0.91}         & \textbf{0.83}         & 0.71                  & 0.77                  & \textbf{0.90}         & \textbf{0.81}         & \textbf{0.85}         & 0.84                         \\ 
\hline
\multirow{11}{*}{\begin{tabular}[c]{@{}c@{}}Test Top-4 \\ NFR (249)\\w/o training~\end{tabular}}      & \textbf{ZSL(Sbert + MultiNFR\_B)}   & \textbf{0.73}                  & \textbf{0.43}         & \uline{0.54}  & 0.69          & \textbf{0.64}         & \textbf{0.66}         & \textbf{0.53}         & 0.71                  & \textbf{0.61}         & \textbf{0.48}         & \textbf{0.57}         & \textbf{0.52}         & \textbf{0.58}                \\
                                                                                                     & ZSL(Sbert + MultiNFR\_D)            & 0.69                           & 0.40                  & 0.51          & 0.65          & 0.53                  & 0.58                  & 0.38                  & 0.23                  & 0.47                  & 0.46                  & 0.53                  & 0.58                  & 0.53                         \\
                                                                                                     & ZSL(AllMini + MultiNFR\_A)          & 0.67                           & 0.36                  & 0.47          & 0.66          & 0.92                  & 0.77                  & 0.33                  & 0.32                  & 0.33                  & 0.45                  & 0.50                  & 0.47                  & 0.51                         \\
                                                                                                     & \textbf{ZSL(AllMini + MultiNFR\_B)} & \textbf{\uline{0.77}}          & 0.36                  & 0.49          & 0.63          & \textbf{\uline{0.94}} & \textbf{\uline{0.76}} & \textbf{\uline{0.64}} & 0.64                  & \textbf{\uline{0.64}} & \textbf{\uline{0.59}} & \textbf{\uline{0.70}} & \textbf{\uline{0.64}} & \uline{\textbf{0.63}}        \\
                                                                                                     & ZSL(AllMini + MultiNFR\_C)          & 0.54                           & 0.45                  & 0.49          & 0.76          & 0.67                  & 0.71                  & 0.36                  & 0.37                  & 0.37                  & 0.41                  & 0.54                  & 0.47                  & 0.51                         \\
                                                                                                     & ZSL(BERT4RE + MultiNFR\_A)          & 0.32                           & 0.09                  & 0.14          & 0.18          & 0.11                  & 0.13                  & 0.33                  & 0.02                  & 0.03                  & 0.19                  & 0.67                  & 0.30                  & 0.14                         \\
                                                                                                     & ZSL(BERT4RE + MultiNFR\_B)          & 0.33                           & 0.60                  & 0.42          & \textit{0.00} & \textit{0.00}         & \textit{0.00}         & 0.28                  & 0.53                  & 0.37                  & 0.13                  & 0.02                  & 0.03                  & 0.21                         \\
                                                                                                     & ZSL(BERT4RE + MultiNFR\_D)          & \textit{0.00}                  & \textit{0.00}         & \textit{0.00} & \textit{0.00} & \textit{0.00}         & \textit{0.00}         & 0.24                  & 0.34                  & 0.38                  & 0.25                  & 0.04                  & 0.06                  & 0.11                         \\
                                                                                                     & , ZSL(SObert + MultiNFR\_A)         & \textit{0.00}                  & \textit{0.00}         & \textit{0.00} & 0.60          & 0.05                  & 0.08                  & 0.22                  & \textbf{\uline{0.71}} & 0.33                  & 0.12                  & 0.09                  & 0.10                  & 0.13                         \\
                                                                                                     & ZSL(SObert + MultiNFR\_B)           & 0.30                           & \textbf{\uline{0.81}} & 0.44          & \textit{0.00} & \textit{0.00}         & \textit{0.00}         & 0.29                  & 0.16                  & 0.21                  & 0.08                  & 0.06                  & 0.07                  & 0.19                         \\
                                                                                                     & ZSL(SObert + MultiNFR\_C)           & 0.31                           & 0.36                  & 0.33          & 0.24          & 0.21                  & 0.22                  & 0.31                  & 0.56                  & 0.40                  & \textit{0.00}         & \textit{0.00}         & \textit{0.00}         & 0.25                         \\
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/LMsSpecs.tex <==
% \usepackage{colortbl}
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}
\centering
\small
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}

\caption{Technical Specifications of the Selected LMs.}
\label{tab:LMs-specs}
  \resizebox{1\textwidth}{!}{
\begin{tabular}{lcccccc} 
\toprule
\multicolumn{1}{c}{\textbf{LM}}             & \textbf{Domain}                                                                                                                                  & \textbf{Layers} & \begin{tabular}[c]{@{}c@{}}\textbf{Hidden }\\\textbf{size}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Attention }\\\textbf{heads}\end{tabular} & \textbf{Vocab size} & \begin{tabular}[c]{@{}c@{}}\textbf{Embedding}\\\textbf{~size}\end{tabular}  \\ 
\hline
%{\cellcolor[rgb]{0.937,0.937,0.937}} 
Sbert   & {\cellcolor[rgb]{0.851,0.851,0.851}}                                                                                                             & 12              & 768                                                                     & 12                                                                          & 30,522              & 128                                                                         \\
%{\cellcolor[rgb]{0.937,0.937,0.937}}
AllMini & \multirow{-2}{*}{{\cellcolor[rgb]{0.851,0.851,0.851}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}c@{}}generic \\\end{tabular}} & 12              & 384                                                                     & 12                                                                          & 30,522              & 512                                                                         \\ 
\hline
%{\cellcolor[rgb]{1,0.949,0.8}}
Bert4RE       & %{\cellcolor[rgb]{1,0.898,0.6}} 
& 12              & 768                                                                     & 6                                                                           & 32,000              & 512                                                                         \\
%{\cellcolor[rgb]{1,0.949,0.8}}
SObert        & \multirow{-2}{*}{%{\cellcolor[rgb]{1,0.898,0.6}}
\begin{tabular}[c]{@{}>{\cellcolor[rgb]{1,0.898,0.6}}c@{}}RE/SE specific\\\end{tabular}}     & 12              & 768                                                                     & 12                                                                          & 82,000              & 512                                                                         \\
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/TaskDesc.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}
\centering
\caption{Classification Tasks Performed in our Study and Corresponding Datasets }
\label{tab:Task_Desc}
  \resizebox{1\textwidth}{!}{
\begin{tabular}{llll} 
\toprule
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Task}\end{tabular}} & \multicolumn{1}{c}{\textbf{Aim}}                                                                                                                     & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Type}\end{tabular}} & \multicolumn{1}{c}{\textbf{Dataset (size)}}                                                        \\ 
\hline
\textit{Task FR/NFR}                                                                                           & \begin{tabular}[c]{@{}l@{}}To detect FRs from NFRs.\end{tabular}                                        & Binary                                                                                              & - PROMISE (625)                                                                                    \\ 
\hline
\multirow{3}{*}{\textit{Task NFR}}                                                                          & \begin{tabular}[c]{@{}l@{}}To detect a specific NFR class (e.g., usability) other NFRs.\end{tabular}                & Binary                                                                                              & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}- Top-NFR PROMISE (249)\\- PROMISE (369-370)\end{tabular}}  \\ 
\cline{2-3}
                                                                                                          & \begin{tabular}[c]{@{}l@{}}To classify NFRs to one NFR class.\end{tabular}                                     & Multi-class                                                                                         &                                                                                                    \\ 
\cline{2-3}
                                                                                                          & \begin{tabular}[c]{@{}l@{}}To classify NFRs into one or more NFR classes.\end{tabular} & Multi-label                                                                                         &                                                                                                    \\ 
\hline
\textit{Task Security}                                                                                           & To detect security requirements.                                                                                                                     & Binary                                                                                              & \begin{tabular}[c]{@{}l@{}}- SeqReq (510) - GPS (176)\\- CPN (210) - ePurse (124)\end{tabular}   \\
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/labelsALL.tex <==
% \usepackage{caption}
% \usepackage{booktabs}

%DONE \hl{TODO: make all terms in the labels lowercase.}
\begin{table}
\centering
\caption{Label configurations for \textit{Task FR/NFR}. }
\label{tab:labelsFRvsNFR}
\resizebox{1\textwidth}{!}{
\begin{tabular}{llll} 
\toprule
\textbf{Label Abbr.}    & \textbf{Label Configuration}                                                                                         & \textbf{FR Label }                                                                                                               & \textbf{NFR Label }                                                                                                                                                                            \\ 
\hline
\textbf{\textit{FR\_A}} & Original 1                                                                                                           & ``functional''                                                                                                                     & ``not about functional''                                                                                                                                                                         \\ 
\hline
\textbf{\textit{FR\_B}} & Expert curated                                                                                                       & \begin{tabular}[c]{@{}l@{}}``functional, system, behavior, \\shall, or must''\end{tabular}                                         & \begin{tabular}[c]{@{}l@{}}''not about functional, system, behavior,\\~shall, or must''\end{tabular}                                                                                             \\ 
\hline
\textbf{\textit{FR\_C}} & \begin{tabular}[c]{@{}l@{}}Word embedding \\(selected from top 20 words) +\\~Expert curated\end{tabular}             & \begin{tabular}[c]{@{}l@{}}``functional, system, behavior, \\shall, must, procedural, structural, \\or characterize''\end{tabular} & \begin{tabular}[c]{@{}l@{}}``not about functional, system, behavior, \\shall, must, procedural, structural, \\or characterize''\end{tabular}                                                     \\ 
\hline
\textbf{\textit{FR\_D}} & Original 2                                                                                                           & ``functional''                                                                                                                     & \begin{tabular}[c]{@{}l@{}}``usability, security, availability, legal, look \& feel,\\scalability, fault tolerance, performance,\\operational, maintainability, or portability''\end{tabular}    \\ 
\hline
\textbf{\textit{FR\_E}} & \begin{tabular}[c]{@{}l@{}}Expert curated +\\~Original 2\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}``functional, system, behavior,\\~shall, or must''\end{tabular}                                         & \begin{tabular}[c]{@{}l@{}}``usability, security, availability, legal, look \& feel,\\scalability, fault tolerance, performance,\\operational, maintainability, or portability''\end{tabular}    \\ 
\hline
\textbf{\textit{FR\_F}} & \begin{tabular}[c]{@{}l@{}}Word embedding \\(selected from top 20 words) +\\Expert curated + Original 2\end{tabular} & \begin{tabular}[c]{@{}l@{}}``functional, system, behavior, \\shall, must, procedural, structural, \\or characterize''\end{tabular} & \begin{tabular}[c]{@{}l@{}}``usability, security, availability, legal, look \& feel, \\scalability, fault tolerance, performance, \\operational, maintainability, or portability'' \hline \end{tabular}  \\

%%%SECURITY CASE
%\multicolumn{4}{c} {\textbf{Task NFR---binary case}}

\hline
\textbf{Usability} \\
\vcell{\textbf{\textit{US\_A}}}        & \vcell{Original 1}                                                                                       & \vcell{``usability''}                                                                                                                                                                                                                                                                                                                                                                    & \vcell{``not about usability''}                                                                                                                                                                                               \\[-\rowheight]
\printcelltop                          & \printcelltop                                                                                                         & \printcelltop                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                               \\
\vcell{\textbf{\textit{US\_B}}}        & \vcell{Expert curated}                                                                                              & \vcell{\begin{tabular}[b]{@{}l@{}}``instructive, easy, helpful, useful, \\learnable, explainable, affordable,\\~intuitive, or understandable''\end{tabular}}                                                                                                                                                                                                                             & \vcell{\begin{tabular}[b]{@{}l@{}}``not about instructive, easy,\\helpful, useful, learnable, \\explainable, affordable, \\intuitive, or understandable''\end{tabular}}                                                       \\[-\rowheight]
\printcelltop                          & \printcelltop                                                                                                         & \printcelltop                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                               \\
\vcell{\textbf{\textit{US\_C}}}        & \vcell{\begin{tabular}[b]{@{}l@{}}Word embedding\\~(selected from top 20 words )\end{tabular}}                             & \vcell{\begin{tabular}[b]{@{}l@{}}``accessibility, aesthetic, contextual,\\experience, satisfaction, HCI, UX, \\questionnaire, ease, or ergonomics''\end{tabular}}                                                                                                                                                                                                                       & \vcell{\begin{tabular}[b]{@{}l@{}}''not about accessibility, aesthetic,\\~contextual, experience, satisfaction,\\HCI, UX, questionnaire, \\ease, or ergonomics''\end{tabular}}                                                \\[-\rowheight]
\printcelltop                          & \printcelltop                                                                                                         & \printcelltop                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                               \\
\vcell{\textbf{\textit{US\_D}}}        & \vcell{\begin{tabular}[b]{@{}l@{}}Word embedding \\(selected from top 20 words) +\\~Original 2\end{tabular}} & \vcell{\begin{tabular}[b]{@{}l@{}}``accessibility, aesthetic, contextual,\\experience, satisfaction, HCI, UX, \\questionnaire, ease, or ergonomics''\end{tabular}}                                                                                                                                                                                                                       & \vcell{\begin{tabular}[b]{@{}l@{}}``security, performance, operational, \\look feel, legal, fault tolerance, \\maintainability, scalability, availability,\\~or portability''\end{tabular}}                                    \\[-\rowheight]
\printcelltop                          & \printcelltop                                                                                                         & \printcelltop                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                               \\
\vcell{\textbf{\textit{US\_E}}}        & \vcell{\begin{tabular}[b]{@{}l@{}}Word embedding \\(selected from top 50 words)\\~+ Original 2\end{tabular}}  & \vcell{\begin{tabular}[b]{@{}l@{}}``accessibility, aesthetic, contextual,\\experience, satisfaction, HCI, UX,\\questionnaire, ease, ergonomics, \\designer, evaluate, multimodal, \\practitioner, prototyping, preference,\\~personalization, suitability, focus, \\clarity, responsiveness, judgement,\\~feel, or helpful''\end{tabular}}                                               & \vcell{\begin{tabular}[b]{@{}l@{}}``security, performance, operational,\\~look feel,~~legal, fault tolerance,\\~maintainability, scalability, availability, \\or portability''\end{tabular}}                                   \\[-\rowheight]
\printcelltop                          & \printcelltop                                                                                                         & \printcelltop                                                                                                                                                                                                                                                                                                                                                                         & \printcelltop                                                                                                                                                                                                               \\ 
\hline
\textbf{Security} \\
\textbf{\textit{SE\_A}}                & Original 1                                                                                               & ''security''                                                                                                                                                                                                                                                                                                                                                                            & ``not about~security''                                                                                                                                                                                                        \\
\textbf{\textit{SE\_B}}                & Expert curated                                                                                                      & ``security, authorization, or protection''                                                                                                                                                                                                                                                                                                                                              & ``not about security, authorization, or protection''                                                                                                                                                                          \\
\textbf{\textit{SE\_C}}                & \begin{tabular}[c]{@{}l@{}}Word embedding~\\(selected from top 20 words)\end{tabular}                                     & \begin{tabular}[c]{@{}l@{}}``vulnerability, securing, protecting, \\protection, cybersecurity, assurance,\\~cyber, countermeasure, threat, privacy,\\~authentication, prevention, or confidentiality''\end{tabular}                                                                                                                                                                     & \begin{tabular}[c]{@{}l@{}}``not about vulnerability, securing, protecting,\\protection,~cybersecurity, assurance,\\~cyber, countermeasure, threat, privacy,\\~authentication, prevention, or confidentiality''\end{tabular}  \\
\textbf{\textit{SE\_D}}                & \begin{tabular}[c]{@{}l@{}}Word embedding\\(selected from top 20 words) +~\\Original 2\end{tabular}          & \begin{tabular}[c]{@{}l@{}}``vulnerability, securing, protecting,\\protection,~cybersecurity, assurance,~\\cyber, countermeasure, threat, privacy,~\\authentication, prevention, or confidentiality''\end{tabular}                                                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}``usability, performance, operational, \\look \& feel, legal, fault \& tolerance,\\~maintainability, scalability, availability, or portability''\end{tabular}                                      \\
\textbf{\textit{SE\_E}}                & \begin{tabular}[c]{@{}l@{}}Word embedding\\(selected from top 50 words)~+ \\Original 2\end{tabular}          & \begin{tabular}[c]{@{}l@{}}``vulnerability, security, protection, cybersecurity, \\assurance, countermeasure, threat, privacy,\\~authentication, prevention, confidentiality, trusted,\\~intrusion, compromise, safety, insecure, defensive, \\breach, proactive, tampering, penetration, policy, phishing, \\vulnerable, authorization, dependability, or certification''\end{tabular} & \begin{tabular}[c]{@{}l@{}}``usability, performance, operational, \\look \& feel, legal, fault \& tolerance, \\maintainability, scalability, availability, or portability''\end{tabular}                                      \\

\bottomrule
\end{tabular}
}
\end{table}

==> Tables/labelsNFRnotfrequent.tex <==


\begin{table}
\caption{Labelling strategies for the NFR task - Part 2.}
\label{tab:labelsNFRnotfrequent2}

\resizebox{1\textwidth}{!}{

\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Labels Group} & \textbf{Labelling Strategy}                                                                                   & \textbf{Non-functional class}                                                                                                                                                                                                                                                                                                                                                                                                             & \textbf{Not about Non-functional class}                                                                                                                                                                                                                                                    \\ \hline
labels\_LF\_A         & Exact "original" labels                                                                                         & "Look \& feel"                                                                                                                                                                                                                                                                                                                                                                                                                            & "not about Look \& feel"                                                                                                                                                                                                                                                                   \\ \hline
labels\_LF\_B         & Expert's curated                                                                                                & "appearance, interface, look \& feel"                                                                                                                                                                                                                                                                                                                                                                                                     & "not about appearance, interface, look \& feel"                                                                                                                                                                                                                                            \\ \hline
                      & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20)\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}"graphical, gui, ui, widget, interaction, \\ habit, prefer, comfortable, friendly, \\ feeling, experience, or familiar"\end{tabular}                                                                                                                                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}" not about graphical, gui, ui, \\ widget, interaction, habit, prefer, \\ comfortable, friendly, feeling, \\ experience, or familiar"\end{tabular}                                                                                                              \\ \hline
labels\_LF\_C         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20) \\ + Exact "original" labels\end{tabular} & \begin{tabular}[c]{@{}l@{}}"graphical, gui, ui, widget, interaction, \\ habit, prefer, comfortable, friendly, \\ feeling, experience, or familiar"\end{tabular}                                                                                                                                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, \\ performance, fault \& tolerance, \\ legal, maintainability, scalability, \\ availability, or portability"\end{tabular}                                                                                                    \\ \hline
labels\_LF\_D         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 50) \\ + Exact "original" labels\end{tabular}  & \begin{tabular}[c]{@{}l@{}}"graphical, gui, ui, widget, interaction, \\ habit, prefer, comfortable, friendly, \\ feeling, experience, familiar, desire, \\ customize, intent, disability, or impression"\end{tabular}                                                                                                                                                                                                                     & as above                                                                                                                                                                                                                                                                                   \\ \hline
labels\_L\_A          & Exact "original" labels                                                                                         & "legal"                                                                                                                                                                                                                                                                                                                                                                                                                                   & "not about legal"                                                                                                                                                                                                                                                                          \\ \hline
labels\_L\_B          & Expert's curated                                                                                                & "legal, law, or rules"                                                                                                                                                                                                                                                                                                                                                                                                                    & "not about legal, law, or rules"                                                                                                                                                                                                                                                           \\ \hline
labels\_L\_C          & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20)\end{tabular}                               & \begin{tabular}[c]{@{}l@{}}"liability, litigation, jurisdiction, regulation, \\ copyright, legislation, enforcement, governmental, \\ directive,civil, right, patentability, claim, violate, \\ infringement, or counsel"\end{tabular}                                                                                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}"not about liability, litigation, \\ jurisdiction, regulation, copyright, \\ legislation, enforcement, governmental, \\ directive,civil, right, patentability, \\ claim, violate, infringement, or counsel"\end{tabular}                                        \\ \hline
labels\_L\_D          & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20) \\ + Exact "original" labels\end{tabular} & \begin{tabular}[c]{@{}l@{}}"liability, litigation, jurisdiction, regulation, \\ copyright, legislation, enforcement, governmental, \\ directive, civil, right, patentability, claim, \\ violate, infringement, or counsel"\end{tabular}                                                                                                                                                                                                   & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, \\ performance, look \& feel, fault \& tolerance, \\ maintainability, scalability, availability, \\ or portability"\end{tabular}                                                                                             \\ \hline
labels\_L\_E          & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 50) \\ + Exact "original" labels\end{tabular}  & \begin{tabular}[c]{@{}l@{}}"liability, litigation, jurisdiction, regulation, \\ copyright, legislation, enforcement, \\ governmental, directive,civil, right, patentability, \\ claim, violate, infringement, counsel, holder, \\ dispute, illegal, judicial, ruling, agreement, \\ ownership, comply, authority, law, accountability, \\ abuse, intellectual, obligation, invention, \\ court, ethical, concern, or policy"\end{tabular} & as above                                                                                                                                                                                                                                                                                   \\ \hline
labels\_FT\_A         & Exact "original" labels                                                                                         & "fault \& tolerance"                                                                                                                                                                                                                                                                                                                                                                                                                      & "not about fault \& tolerance"                                                                                                                                                                                                                                                             \\ \hline
labels\_FT\_B         & Expert's curated                                                                                                & "system recovery \& fault tolerance"                                                                                                                                                                                                                                                                                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}"not about system recovery \& \\ fault tolerance"\end{tabular}                                                                                                                                                                                                  \\ \hline
labels\_FT\_C         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20)\end{tabular}                               & \begin{tabular}[c]{@{}l@{}}"tolerance, failure, tolerant, byzantine, \\ deadlock, exploiting, reliability, \\ isolation, fault, guarantee, or dependable"\end{tabular}                                                                                                                                                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}"not about tolerance, failure, tolerant, \\ byzantine, deadlock, exploiting, \\ reliability, isolation, fault, guarantee, \\ dependable, countermeasure, resilience, \\ defensive, corruption, weakness, \\ malfunction, robustness, or stability"\end{tabular} \\ \hline
                      & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20) \\ + Exact "original" labels\end{tabular}  & \begin{tabular}[c]{@{}l@{}}"tolerance, failure, tolerant, byzantine, \\ deadlock, exploiting, reliability, isolation, \\ fault, guarantee, dependable, countermeasure, \\ resilience, defensive, corruption, \\ weakness, malfunction, robustness, or stability"\end{tabular}                                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, \\ performance, look \& feel, legal, \\ maintainability, scalability, \\ availability, or portability"\end{tabular}                                                                                                          \\ \hline
labels\_FT\_D         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 50) \\ + Exact "original" labels\end{tabular}  & \begin{tabular}[c]{@{}l@{}}"tolerance, failure, tolerant, byzantine, \\ deadlock, exploiting, reliability, isolation, \\ fault, guarantee, dependable, countermeasure, \\ resilience, defensive, corruption, weakness, \\ malfunction, robustness, or stability"\end{tabular}                                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}"performance, look \& feel, legal, \\ maintainability, scalability, availability, \\ or portability"\end{tabular}                                                                                                                                               \\ \hline
labels\_MN\_A         & Exact "original" labels                                                                                         & "maintainability"                                                                                                                                                                                                                                                                                                                                                                                                                         & "not about maintainability"                                                                                                                                                                                                                                                                \\ \hline
labels\_MN\_B         & Expert's curated                                                                                                & "maintaining, fixing, running or updating"                                                                                                                                                                                                                                                                                                                                                                                                & \begin{tabular}[c]{@{}l@{}}"not about maintaining, fixing, \\ running or updating"\end{tabular}                                                                                                                                                                                            \\ \hline
labels\_MN\_C         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20)\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}"adaptability, effectiveness, \\ agility, preventive, or dependability"\end{tabular}                                                                                                                                                                                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}"not about adaptability, effectiveness, \\ agility, preventive, or dependability"\end{tabular}                                                                                                                                                                  \\ \hline
labels\_MN\_D         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20) \\ + Exact "original" labels\end{tabular} & \begin{tabular}[c]{@{}l@{}}"adaptability, effectiveness, \\ agility, preventive, or dependability"\end{tabular}                                                                                                                                                                                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, \\ performance, look \& feel, legal, \\ fault \& tolerance, scalability, availability, \\ or portability"\end{tabular}                                                                                                       \\ \hline
labels\_MN\_E         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 50) \\ + Exact "original" labels\end{tabular} & \begin{tabular}[c]{@{}l@{}}"adaptability, effectiveness, agility, \\ preventive, dependability, correcting, \\ reuse, defect, mitigation, validated, \\ resilience, achievable, remedy, \\ assessing, or maintaining"\end{tabular}                                                                                                                                                                                                        & as above                                                                                                                                                                                                                                                                                   \\ \hline

\end{tabular}
}
\caption{Labelling strategies for the NFR task - Part 1.}
\label{tab:labelsNFRnotfrequent1}
\end{table}




\begin{table}

\resizebox{1\textwidth}{!}{

\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Labels Group} & \textbf{Labelling Strategy}                                                                                   & \textbf{Non-functional class}                                                                                                                                                                                                                                                                                                                                                                                                             & \textbf{Not about Non-functional class}                                                                                                                                                                                                                                                    \\ \hline

labels\_SC\_A         & Exact "original" labels                                                                                         & "scalability"                                                                                                                                                                                                                                                                                                                                                                                                                             & "not about scalability"                                                                                                                                                                                                                                                                    \\ \hline
labels\_SC\_B         & Expert's curated                                                                                                & "scalable, increasable or developable"                                                                                                                                                                                                                                                                                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}"not about scalable, \\ increasable or developable"\end{tabular}                                                                                                                                                                                                \\ \hline
labels\_SC\_C         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20)\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}"flexibility, workload, efficiency, \\ or optimize"\end{tabular}                                                                                                                                                                                                                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}"not about flexibility, workload, \\ efficiency, or optimize"\end{tabular}                                                                                                                                                                                      \\ \hline
labels\_SC\_D         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20) \\ + Exact "original" labels\end{tabular} & \begin{tabular}[c]{@{}l@{}}"flexibility, workload, efficiency, \\ or optimize"\end{tabular}                                                                                                                                                                                                                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, \\ performance, look \& feel, legal, \\ fault \& tolerance, maintainability, \\ availability, or portability"\end{tabular}                                                                                                   \\ \hline
labels\_SC\_E         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 50) \\ + Exact "original" labels\end{tabular} & \begin{tabular}[c]{@{}l@{}}"flexibility, workload, efficiency, optimize, \\ caching, improvement, robust, overhead, \\ adaptability, scalable, or increased"\end{tabular}                                                                                                                                                                                                                                                                 & as above                                                                                                                                                                                                                                                                                   \\ \hline
labels\_A\_A          & Exact "original" labels                                                                                         & "availability"                                                                                                                                                                                                                                                                                                                                                                                                                            & "not about availability"                                                                                                                                                                                                                                                                   \\ \hline
labels\_A\_B          & Expert's curated                                                                                                & "avaliable or timely achievable"                                                                                                                                                                                                                                                                                                                                                                                                          & \begin{tabular}[c]{@{}l@{}}"not about avaliable \\ or timely achievable"\end{tabular}                                                                                                                                                                                                      \\ \hline
labels\_A\_C          & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20)\end{tabular}                              & "reliability, dependability, resilience"                                                                                                                                                                                                                                                                                                                                                                                                  & \begin{tabular}[c]{@{}l@{}}"not about reliability, dependability, \\ resilience"\end{tabular}                                                                                                                                                                                              \\ \hline
labels\_A\_D          & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20) \\ + Exact "original" labels\end{tabular} & "reliability, dependability, resilience"                                                                                                                                                                                                                                                                                                                                                                                                  & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, \\ performance, look \& feel, legal, \\ fault \& tolerance, maintainability, \\ scalability, or portability"\end{tabular}                                                                                                    \\ \hline
labels\_A\_E          & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 50) \\ + Exact "original" labels\end{tabular} & \begin{tabular}[c]{@{}l@{}}"reliability, dependability, resilience, \\ flexibility, accountability, ensure, disruption, \\ timely, or standby"\end{tabular}                                                                                                                                                                                                                                                                               & as above                                                                                                                                                                                                                                                                                   \\ \hline
labels\_PO\_A         & Exact "original" labels                                                                                         & "portability"                                                                                                                                                                                                                                                                                                                                                                                                                             & "not about portability"                                                                                                                                                                                                                                                                    \\ \hline
labels\_PO\_B         & Expert's curated                                                                                                & "portable or transferable"                                                                                                                                                                                                                                                                                                                                                                                                                & "not about portable or transferable"                                                                                                                                                                                                                                                       \\ \hline
labels\_PO\_C         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20)\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}"porting, portable, compatibility, \\ interoperability, or standalone"\end{tabular}                                                                                                                                                                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}"not about porting, portable, c\\ ompatibility, interoperability, or standalone"\end{tabular}                                                                                                                                                                   \\ \hline
labels\_PO\_D         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 20) \\ + Exact "original" labels\end{tabular} & \begin{tabular}[c]{@{}l@{}}"porting, portable, compatibility, \\ interoperability, or standalone"\end{tabular}                                                                                                                                                                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}"usability, security, operational, \\ performance, look \& feel, legal, \\ fault \& tolerance, maintainability, \\ scalability, or availability"\end{tabular}                                                                                                   \\ \hline
labels\_PO\_E         & \begin{tabular}[c]{@{}l@{}}Word Embedding \\ (Selected words top 50) \\ + Exact "original" labels\end{tabular} & \begin{tabular}[c]{@{}l@{}}"porting, portable, compatibility, \\ interoperability, standalone, packaged, \\ lightweight, modularity, wrapper, or installing"\end{tabular}                                                                                                                                                                                                                                                                 & as above                                                                                                                                                                                                                                                                                   \\ \hline

\end{tabular}
}

\end{table}

==> Tables/resultsdetailBinaryNFR_SMALL.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}
\centering
\scriptsize
\caption{Binary classification results of the top 4 NFR classes in \textit{Task NFR}.}
\label{tab:resultsdetailNFRbin}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|l|ccc|ccc} 
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{NFR class (249)}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{ZSL classifier}}} & \multicolumn{3}{c|}{\textbf{NFR class}}       & \multicolumn{3}{c}{\textbf{``Other'' class}}  \\ 
\cline{3-8}
\multicolumn{1}{c|}{}                                         & \multicolumn{1}{c|}{}                                         & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1}     \\ 
\hline
\textbf{US (67)}                                              & Sbert + US\_E                                                 & \textbf{0.73}  & 0.49          & 0.59           & 0.83           & \textbf{0.93} & \textbf{0.88}      \\
\textbf{SE (66)}                                              & AllMini + SE\_D                                               & 0.67           & \textbf{0.73} & \textbf{0.70}  & \textbf{0.90}  & 0.87          & \textbf{0.89}      \\
\textbf{O (62)}                                               & Bert4RE + O\_C                                                & 0.46           & 0.37          & 0.41           & 0.80           & 0.86          & 0.83               \\
\textbf{PE (54)}                                              & Sbert + PE\_E                                                 & 0.50           & 0.46          & 0.48           & 0.85           & 0.87          & 0.86               \\
\textbf{PE (54)}                                              & AllMini + PE\_B                                               & 0.47           & 0.63          & 0.54           & 0.89           & 0.81          & 0.84               \\
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/resultsdetailFRvsNFR_SMALL.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}[t]
\centering
\scriptsize
\caption{Classification results for FR and NFR classes on \textit{Task FR/NFR}, obtained from the best combination for each LM and label configuration.}
\label{tab:resultsFRvsNFRdet}

\begin{tabular}{l|lll|lll} 
\toprule
\multirow{2}{*}{\textbf{ZSL Classifier}} & \multicolumn{3}{l|}{\textbf{FR (255)}} & \multicolumn{3}{l}{\textbf{NFR (370)}}  \\ 
\cline{2-7}
                                              & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1}     \\ 
\hline
\textbf{Sbert + FR\_E}                        & \textbf{0.55}  & \textbf{0.82} & \textbf{0.66} & \textbf{0.82}  & 0.54          & 0.65              \\
AllMini + FR\_D                               & 0.50           & 0.71          & 0.58          & 0.72           & 0.50          & 0.59              \\
Bert4RE + FR\_D                               & 0.47           & 0.65          & 0.54          & 0.67           & 0.50          & 0.57              \\
\textbf{SObert + FR\_C}                       & 0.50           & 0.41          & 0.45          & 0.64           & \textbf{0.72} & \textbf{0.68}     \\
\bottomrule
\end{tabular}

\end{table}
